Spectroscopic orbits of nearby stars

We observed stars with variable radial velocities to determine their spectroscopic orbits. Velocities of 132 targets taken over a time span reaching 30 years are presented. They were measured with the correlation radial velocity spectrometers (1913 velocities) and the new VUES echelle spectrograph (632 velocities), with typical accuracy of 0.5 and 0.2 km/s, respectively. We derived spectroscopic orbits of 57 stars (including 53 first-time orbits), mostly nearby dwarfs of spectral types K and M. Their periods range from 2.2 days to 14 years, some of those are Hipparcos astrometric binaries. Comments on individual objects are provided. Many stars belong to hierarchical systems containing three or more components, including 20 new hierarchies resulting from this project. The preliminary orbit of the young star HIP~47110B has a large eccentricity e=0.47 despite short period of 4.4 d; it could be still circularizing. Our results enrich the data on nearby stars and contribute to a better definition of the multiplicity statistics.

==> listsb1.tex <==
BD+33 4827D & 67.9618 & 51794.504 & 0.197 & 280.4 & 10.263 & \ldots & $-$23.478&  0.58   & $>$0.2  \\
         & $\pm$0.0035 & $\pm$0.633 & $\pm$0.010 & $\pm$3.6 & $\pm$0.125 & \ldots & $\pm$0.080&   \ldots   &  \ldots \\
HIP 3428 & 97.250 & 58183.305 & 0.391 & 21.6 & 25.244 & 26.490 & $-$6.648&   0.52  &  0.56 \\
         & $\pm$0.015 & $\pm$0.266 & $\pm$0.005 & $\pm$1.1 & $\pm$0.197 & $\pm$0.211 & $\pm$0.072& 0.46  & 0.53 \\
HD 8691 & 581.17 & 55965.5 & 0.544 & 313.5 & 2.366 & \ldots & $-$36.183&  0.54   & $>$0.08  \\
         & $\pm$1.21 & $\pm$5.1 & $\pm$0.036 & $\pm$5.5 & $\pm$0.110 & \ldots & $\pm$0.065&   \ldots  & \ldots  \\
HIP 9867 & 897.0 & 56004.0 & 0.0 & 0.0 & 8.057 & 11.347 & 61.419  &  0.38   & 0.40 \\
         & $\pm$2.3 & $\pm$5.8 & fixed & fixed & $\pm$0.114 & $\pm$0.184 & $\pm$0.079& 0.37    & 0.28  \\
HIP 10258 & 5.88554 & 54206.1875 & 0.0   & 0.0 & 66.011 & 64.231 & $-$59.148&  0.92   &  0.66 \\
         & $\pm$0.00001 & $\pm$0.0022 & fixed & fixed & $\pm$0.176 & $\pm$0.189 & $\pm$0.085& 0.88    & 0.68 \\
HIP 13460 Aa,Ab & 76.433  & 58410.20 & 0.057      & 124.1     & 14.565      & 16.060     &  \ldots & 0.88    & 0.12 \\
         & $\pm$0.014  & $\pm$3.20   & $\pm$0.016 & $\pm$14.2 & $\pm$0.254  & $\pm$1.508 &  \ldots & 3.23    & 0.11 \\
HIP 13460 AB & 1862: & 55433    & 0.502      & 232.8    & 4.00      & \ldots & $-$74.386  & \ldots    & $>$0.29  \\
         & $\pm$25  & $\pm$149 & $\pm$0.186 & $\pm$7.4 & $\pm$2.04 & \ldots & $\pm$0.577 &  \ldots   & \ldots  \\
HIP 14478 & 1325.2 & 57011.8 & 0.369 & 142.4 & 5.814 & \ldots & $-$50.871&  0.22   & $>$0.34  \\
         & $\pm$7.8 & $\pm$16.5 & $\pm$0.033 & $\pm$5.8 & $\pm$0.162 & \ldots & $\pm$0.183&   \ldots   &  \ldots \\
HIP 14864 & 59.428 & 56470.94 & 0.642           & 130.3   & 27.626    & 31.667      & $-$31.907&  0.37   & 0.33 \\
         & $\pm$0.005 & $\pm$0.07 & $\pm$0.006 & $\pm$0.8 & $\pm$0.256 & $\pm$1.020 & $\pm$0.138&  1.15   & 0.29 \\
HIP 17102 & 183.113  & 57305.62   & 0.6115         & 350.09    & 25.134     & 24.121    &  4.273     & 0.42    & 0.56  \\
         & $\pm$0.019  & $\pm$0.17    & $\pm$0.0020& $\pm$0.49 & $\pm$0.124 &$\pm$0.128 & $\pm$0.073 & 0.41    & 0.58 \\
HIP 18448 & 1538.9 & 54793.6 & 0.478 & 210.6 & 6.469 & \ldots & 16.657&   0.34  & $>$0.38 \\
         & $\pm$2.6 & $\pm$5.9 & $\pm$0.018 & $\pm$2.3 & $\pm$0.117 & \ldots & $\pm$0.088&   \ldots   &  \ldots \\
HIP 19915 & 7.30032 & 50087.8789 & 0.0 & 0.0 & 27.326 & 30.620 & $-$8.157&  1.25   & 0.078 \\
         & $\pm$0.00003 & $\pm$0.0092 & fixed & fixed & $\pm$0.160 & $\pm$0.182 & $\pm$0.107& 1.44    & 0.069 \\
HD 279846 & 15.4860 & 55271.598 & 0.039 & 245.1 & 44.723 & 47.041 & 12.429&  0.78   &  0.63 \\
         & $\pm$0.0001 & $\pm$0.189 & $\pm$0.003 & $\pm$4.5 & $\pm$0.217 & $\pm$0.225 & $\pm$0.075&  1.09   & 0.60 \\
HIP 20709 & 140.748 & 56222.61 &  0.557       & 280.0     & 23.200    & 31.750      & 44.060 &  0.19   &  0.84 \\
         & $\pm$0.020 & $\pm$0.34 & $\pm$0.007 & $\pm$0.6 & $\pm$0.086 & $\pm$0.332 & $\pm$0.067 &  0.19   & 0.60 \\
HIP 21710 & 610.43 & 56635.1 & 0.415         & 269.9    & 4.596 & \ldots & $-$27.124  &  0.75   & $>$0.17  \\
         & $\pm$0.15 & $\pm$4.2 & $\pm$0.018 & $\pm$3.4 & $\pm$0.099 & \ldots & $\pm$0.067&   \ldots   &  \ldots \\
HIP 28663 & 8.5542 & 52158.14 & 0.079 & 255.3 & 30.129 & \ldots & $-$25.105&  0.68   &  $>$0.35 \\
         & $\pm$0.0001 & $\pm$0.12 & $\pm$0.006 & $\pm$5.0 & $\pm$0.229 & \ldots & $\pm$0.136&   \ldots   &  \ldots \\
HIP 34341 & 875.37 & 55875.7 & 0.507 & 328.7 & 4.561 & \ldots & $-$17.353&  0.45   &  $>$0.20\\
         & $\pm$1.69 & $\pm$8.6 & $\pm$0.026 & $\pm$5.4 & $\pm$0.284 & \ldots & $\pm$0.106&   \ldots   & \ldots  \\
HIP 35706 & 4741 & 56641 & 0.337 & 266.5 & 5.639 & \ldots & $-$29.953&  0.22   & $>$0.57  \\
         & $\pm$73 & $\pm$41 & $\pm$0.022 & $\pm$4.6 & $\pm$0.098 & \ldots & $\pm$0.125&   \ldots   &  \ldots \\
HIP 39681 & 1717.7 & 51745.8 & 0.508 & 76.3 & 8.077 & \ldots & $-$0.569& 0.47    & $>$0.51  \\
         & $\pm$0.7 & $\pm$3.7 & $\pm$0.009 & $\pm$1.5 & $\pm$0.116 & \ldots & $\pm$0.054&  \ldots    &  \ldots \\
HIP 40253& 897.83 & 54881 & 0.035 & 340 & 6.638 & \ldots & $-$3.255&  0.51   & $>$0.37  \\
         & $\pm$0.86 & $\pm$66 & $\pm$0.010 & $\pm$26.5 & $\pm$0.151 & \ldots & $\pm$0.060&   \ldots   & \ldots  \\
HD 71028 & 1129.5 & 53846.9 & 0.147 & 166.1 & 4.989 & \ldots & 34.147&  0.41   & $>$0.29  \\
         & $\pm$3.2 & $\pm$42.6 & $\pm$0.028 & $\pm$14.2 & $\pm$0.174 & \ldots & $\pm$0.086&   \ldots   &  \ldots \\
HIP 46383 & 8.490802 & 57396.839      & 0.0987     & 324.3     & 56.286 & 57.002 & $-$32.322        & 0.38     & 0.63 \\
         & $\pm$0.000003 & $\pm$0.013 & $\pm$0.0016 & $\pm$0.6 & $\pm$0.095 & $\pm$0.096 & $\pm$0.005& 0.43    & 0.63 \\
HIP 46926 & 3.10662 & 54604.7305 & 0.0 & 0.0 & 22.600 & 26.464 & $-$10.859&  0.59   & 0.020 \\
         & $\pm$0.00001   & $\pm$0.0025 & fixed & fixed & $\pm$0.127 & $\pm$0.185 & $\pm$0.065& 0.50    & 0.017 \\
HIP 47133 & 4.38804 & 58055.344 & 0.474 & 140.2 & 69.252 & 74.379 & $-$0.677&  2.71   &  0.47 \\
         & $\pm$0.00001 & $\pm$0.015 & $\pm$0.005 & $\pm$1.9 & $\pm$2.035 & $\pm$2.506 & $\pm$0.257&  2.79   &  0.44 \\
HIP 47899 & 146.309 & 56614.18 & 0.075 & 5.8 & 20.100 & 21.360 & $-$15.010&  0.66   & 0.55 \\
         & $\pm$0.020 & $\pm$1.50 & $\pm$0.005 & $\pm$3.6 & $\pm$0.131 & $\pm$0.144 & $\pm$0.071& 0.63    & 0.52 \\
HIP 48346  & 79.013 & 56464.52 & 0.695        & 187.9     & 26.408     & 36.202     & $-$14.648&  0.86   &  0.43 \\
         & $\pm$0.073 & $\pm$1.03 & $\pm$0.041 & $\pm$2.5 & $\pm$3.209 & $\pm$4.602 & $\pm$0.308&  2.82   & 0.31 \\
HIP 50156 & 73.225 & 56288.11 & 0.140 & 308.7 & 9.851 & \ldots & 8.741&   0.63  & $>$0.22  \\
         & $\pm$0.030 & $\pm$2.10 & $\pm$0.027 & $\pm$11.1 & $\pm$0.266 & \ldots & $\pm$0.222&  \ldots   & \ldots \\
HIP 50271  & 47.4632 & 49595.278 & 0.688 & 55.6 & 28.703 & \ldots & 4.288&  0.98   & $>$0.45  \\
         & $\pm$0.0003 & $\pm$0.028 & $\pm$0.003 & $\pm$0.6 & $\pm$0.156 & \ldots & $\pm$0.108&  \ldots   & \ldots \\
HIP 56229 & 186.3:  & 58096.59 & 0.549 & 345.7 & 22.183 & 23.033 & 12.015&  0.42   & 0.53 \\
         & $\pm$0.73 & $\pm$1.04 & $\pm$0.050 & $\pm$1.7 & $\pm$2.298 & $\pm$2.386 & $\pm$0.064&  0.33   & 0.51 \\
HIP 57058 &  725.9 & 57934.3         & 0.164 & 168.0    &   8.065 & \ldots & 19.708& 0.53    & $>$0.50  \\
         & $\pm$0.9 & $\pm$61.7 & $\pm$0.079 & $\pm$28.9 & $\pm$1.128 & \ldots & $\pm$0.603& \ldots    & \ldots \\
BD+44 2120B & 2.22596 & 55870.6875 & 0.0 & 0.0 & 46.215 & \ldots & $-$4.387&  1.15   & $>$0.35  \\
         & $\pm$0.00001  & $\pm$0.0038 & fixed & fixed & $\pm$0.322 & \ldots & $\pm$0.218& \ldots    &\ldots  \\
HIP 61436 & 299.55 & 56819.02 & 0.457 & 260.7 & 17.590 & 19.677 & $-$0.363&  0.48   & 0.49 \\
         & $\pm$0.18 & $\pm$1.24 & $\pm$0.013 & $\pm$1.9 & $\pm$0.294 &  $\pm$0.491 & $\pm$0.135& 0.96    & 0.46 \\
HIP 62755 & 2238 & 56347.9 & 0.140 & 27.3 & 8.027 & \ldots & $-$47.032& 0.11    & $>$0.69 \\
         & $\pm$27 & $\pm$127.6 & $\pm$0.024 & $\pm$20.9 & $\pm$0.419 & \ldots & $\pm$0.167&   \ldots  & \ldots \\
HIP 65026 & 446.87 & 57009.7      & 0.082     & 12.2     & 9.129      & \ldots & 0.109&   0.65  & 0.65: \\
         & $\pm$0.43 & $\pm$10.1 & $\pm$0.014 & $\pm$8.4 & $\pm$0.158 & \ldots & $\pm$0.104& \ldots  & $>$0.29   \\
HIP 65327 & 4354.0 & 56827.0 & 0.497          & 115.2    & 5.030      & \ldots & $-$8.528  &  0.21   & $>$0.45  \\
         & $\pm$13.8 & $\pm$55.8 & $\pm$0.051 & $\pm$8.7 & $\pm$0.557 & \ldots & $\pm$0.20 &  \ldots   & \ldots \\
HIP 65887 & 1200.0 & 53733.7 & 0.078 & 68.6 & 6.143 & \ldots & $-$3.416&  0.45   & $>$0.38  \\
         & $\pm$3.0 & $\pm$47.8 & $\pm$0.020 & $\pm$14.5 & $\pm$0.134 & \ldots & $\pm$0.074&  \ldots   & \ldots \\
HIP 66290 & 1967 & 51294.7 & 0.681 & 78.5 & 6.731 & \ldots & $-$14.044&  0.54   & $>$0.36  \\
         & $\pm$11 & $\pm$9.1 & $\pm$0.018 & $\pm$5.8 & $\pm$0.315 & \ldots & $\pm$0.139& \ldots    &\ldots  \\
HIP 67086 & 40.871    & 56774.02   & 0.318      & 208.9    & 28.116     & 33.602     & $-$27.226  &  0.55   & 0.46     \\
         & $\pm$0.007  & $\pm$0.34 & $\pm$0.024 & $\pm$2.8 & $\pm$0.564 & $\pm$1.070  & $\pm$0.255 &  0.54   & 0.39   \\
BD+26 2498 & 1536.2 & 53208.1 & 0.190 & 258.3 & 12.063 & \ldots & $-$13.641&  0.52   & $>$1.02  \\
         & $\pm$1.8 & $\pm$15.0 & $\pm$0.010 & $\pm$3.5 & $\pm$0.117 & \ldots & $\pm$0.100&   \ldots  &\ldots  \\
BD+19 2735 & 3616 & 55769.8 & 0.607 & 89.8 & 4.913 & \ldots & $-$9.535& 0.28    &  $>$0.34 \\
         & $\pm$69 & $\pm$33.2 & $\pm$0.176 & $\pm$7.9 & $\pm$1.566 & \ldots & $\pm$0.120&  \ldots   & \ldots \\
HIP 68801 & 2.84019 & 54536.9453 & 0.0 & 0.0 & 86.676 & 88.273 & $-$36.319& 1.10    & 0.79 \\
         & $\pm$0.00001 & $\pm$0.0009 & fixed & fixed & $\pm$0.173 & $\pm$0.222 & $\pm$0.099& 0.90    & 0.78 \\
HIP 69549 & 6.03150 & 54087.0820 & 0.0 & 0.0 & 64.754 & 65.831 & 8.578&  1.13   & 0.70 \\
         & $\pm$0.00001 & $\pm$0.0016 & fixed & fixed & $\pm$0.132 & $\pm$0.139 & $\pm$0.068& 1.36    & 0.69 \\
HIP 76941 & 267.06   & 57157.05  & 0.492      & 315.3    & 7.054     & \ldots & $-$12.497  &  0.38   & $>$0.23  \\
         & $\pm$0.31 & $\pm$1.36 & $\pm$0.012 & $\pm$1.7 & $\pm$0.122 & \ldots & $\pm$0.071&  \ldots   & \ldots \\
HIP 77141 & 17.3120 & 58299.184 & 0.836 & 14.2 & 50.441 & \ldots & $-$3.460&  0.28   & $>$0.34  \\
         & $\pm$0.0005 & $\pm$0.070 & $\pm$0.154 & $\pm$8.1 & $\pm$58.975 & \ldots & $\pm$2.167& \ldots    & \ldots \\
HIP 78158 & 322.04 & 57083.48 & 0.395 & 299.7 & 11.784 & \ldots & $-$44.839&  0.34   & $>$0.44 \\
         & $\pm$0.16 & $\pm$1.43 & $\pm$0.014 & $\pm$1.9 & $\pm$0.219 & \ldots     & $\pm$0.099&  \ldots   & \ldots \\
%HIP 79796 & 1.5736 & 2004.8700 & 0.246 & 21.9 & 10.320 & 17.470 & $-$34.880& 0.34    &  \\
%         & $\pm$0 !!! & fixed & fixed & fixed & fixed & fixed & fixed&     &  \\
HIP 80751 & 5252 & 58096.9 & 0.188 & 64.5 & 3.031 & \ldots & $-$32.748&  0.23   &   $>$1.02  \\
         & $\pm$324 & $\pm$692.7 & $\pm$0.069 & $\pm$55.1 & $\pm$0.748 & \ldots & $\pm$0.582&   \ldots  & \ldots \\
HIP 92952 & 7.9461 & 57609.65 & 0.044 & 291.9 & 17.290 & \ldots & $-$18.380&  0.40   & $>$0.18  \\
         & $\pm$0.0002 & $\pm$0.28 & $\pm$0.007 & $\pm$12.8 & $\pm$0.148 & \ldots & $\pm$0.133& \ldots    & \ldots \\
BD+77 767 & 17.3231 & 56737.1289 & 0.391 & 225.5 & 40.434 & \ldots & $-$25.831&  0.32   & $>$0.63 \\
         & $\pm$0.0002 & $\pm$0.0329 & $\pm$0.005 & $\pm$0.9 & $\pm$0.331 & \ldots & $\pm$0.114&  \ldots   &\ldots  \\
HIP 101941 & 1026.69 & 54442.6 & 0.223 & 211.8 & 9.975 & \ldots & $-$20.562& 0.43    & $>$0.64  \\
         & $\pm$1.37 & $\pm$7.8 & $\pm$0.012 & $\pm$2.8 & $\pm$0.111 & \ldots & $\pm$0.075&   \ldots  & \ldots \\
HIP 102320 & 21.1854 & 57143.617 & 0.416 & 322.1 & 40.879 & 41.954 & $-$21.080&  0.30   & 0.47 \\
         & $\pm$0.0002 & $\pm$0.016 & $\pm$0.003 & $\pm$0.3 & $\pm$0.141 & $\pm$0.206 & $\pm$0.049& 0.19    & 0.46 \\
HIP 104994 & 51.82128 & 55970.823 & 0.407       & 303.6     & 25.796     & 32.988     & $-$46.869&  0.85   &  0.48\\
         & $\pm$0.0015 & $\pm$0.087 & $\pm$0.003 & $\pm$0.9 & $\pm$0.090 & $\pm$0.152 & $\pm$0.062&  0.49   & 0.37 \\
HIP 110291    & 764.8 & 54423.0 & 0.563 & 3.9 & 3.888 & \ldots & $-$108.035& 0.52    & $>$0.15  \\
          & $\pm$3.5 & $\pm$4.7 & $\pm$0.028 & $\pm$4.0 & $\pm$0.219 & \ldots & $\pm$0.088& \ldots    & \ldots \\
HIP 111685 & 6177 & 54730 & 0.249 & 300.1 & 3.752 & \ldots & $-$58.378&  0.33   & $>$0.40  \\
         & $\pm$26 & $\pm$22 & $\pm$0.007 & $\pm$1.3 & $\pm$0.154 & \ldots & $\pm$0.113&  \ldots   & \ldots \\
HIP 111942 & 375.098  & 56849.88  & 0.437      & 339.5   & 7.880 & \ldots & $-$32.470   &  0.32   & $>$0.30  \\
         & $\pm$0.038 & $\pm$1.39 & $\pm$0.011 & $\pm$0.4 & $\pm$0.080 & \ldots & $\pm$0.070&  \ldots   & \ldots \\
HIP 112523 & 3255: & 55676.2 & 0.480 & 190.5 & 3.871 & \ldots & 4.154&  0.58   & $>$0.36  \\
         & $\pm$50 & $\pm$41.7 & fixed & $\pm$6.2 & $\pm$0.243 & \ldots & $\pm$0.156&  \ldots   & \ldots \\
BD+66 1664 & 3.09995 & 53785.0117 & 0.0 & 0.0 & 23.940 & \ldots & $-$22.083& 0.67    & $>$0.18  \\
         & $\pm$0.00004 & $\pm$0.0036 & fixed & fixed & $\pm$0.174 & \ldots & $\pm$0.123&  \ldots   & \ldots \\
HIP 118212 & 872.90 & 56678.80   & 0.536      & 135.4    & 8.428     & \ldots  & 0.999&  0.36   & $>$0.40  \\
         & $\pm$1.23 & $\pm$2.71 & $\pm$0.016 & $\pm$2.5 & $\pm$0.138 & \ldots & $\pm$0.131& \ldots    &\ldots  \\


==> stattable.tex <==
HIP 96       &  00 01 13.19 &  $+$13 58 30.3 & 10.59 &   23.25 & M0.5  & V  &   7 &   2555 &    $-$7.93 &   1.49 &   23.6  \\
BD+13 5195B  &  00 01 12.87 &  $+$13 58 19.7 & 11.12 &   27.77 & M1    & V  &   5 &   2541 &   $-$10.15 &   0.82 &   10.4  \\
HIP 374      &  00 04 40.08 &  $+$34 15 54.4 &  7.08 &    5.64 & K0    & C  &   4 &   6231 &   $-$24.02 &   0.35 &    1.8  \\
HIP 375      &  00 04 40.19 &  $+$34 16 19.8 & 10.13 &    1.00 & --    &  C &   4 &   6242 &    $-$9.17 &   0.24 &    0.9  \\
BD+33 4827D  &  00 04 33.54 &  $+$34 15 03.5 & 10.55 &    4.56 & F9    & S1 &  49 &   6242 &   $-$23.48 & \ldots & \ldots  \\
HIP 1412     &  00 17 40.90 &  $-$08 40 56.2 & 10.95 &   31.57 & K7V   & V  &   6 &   1479 &    15.73 &  14.41 &   99.0  \\
HIP 3428     &  00 43 41.42 &  $+$23 53 07.1 & 10.97 &   22.18 & K7    & S2 &  16 &   2168 &    $-$6.65 & \ldots & \ldots  \\
HIP 5110A    &  01 05 29.92 &  $+$15 23 24.2 &  9.17 &   36.65 & K3.5V & C  &   4 &   2915 &    $-$5.72 &   0.35 &    2.4  \\
HD 6440B     &  01 05 29.76 &  $+$15 23 15.5 &  9.93 &   37.41 & K8V   & V  &   8 &   2915 &    $-$3.22 &   1.23 &   12.7  \\
HD 8691      &  01 26 09.28 &  $+$31 54 52.6 &  9.24 &   19.96 & G0    & S1 &  42 &   5440 &   $-$36.18 & \ldots & \ldots  \\
HIP 9867     &  02 06 57.21 &  $+$45 11 04.1 & 10.24 &   51.47 & M0V   & S2 &  17 &   5479 &    61.42 & \ldots & \ldots  \\
HIP 10258    &  02 11 57.98 &  $+$04 21 41.8 &  9.72 &   21.36 & K5    & S2 &  30 &   4742 &   $-$59.15 & \ldots & \ldots  \\
BD+49 646    &  02 22 33.89 &  $+$50 33 36.9 &  9.65 &   18.91 & --    & s2 &   8 &   4711 &   $-$10.00 & \ldots & \ldots  \\
HIP 11437    &  02 27 29.25 &  $+$30 58 24.6 & 10.12 &   24.36 & K7V   & C  &  10 &   5884 &     5.98 &   0.46 &    1.8  \\
HIP 12787    &  02 44 21.36 &  $+$10 57 41.3 & 11.10 &   20.51 & M0Ve  & s2 &  12 &   2970 &     4.20 & \ldots & \ldots  \\
HIP 13398    &  02 52 25.03 &  $+$26 58 29.9 & 11.05 &   42.67 & M2V   & V? &  13 &   5459 &   $-$11.59 &   0.74 &    3.7  \\
HIP 13460    &  02 53 18.50 &  $+$60 51 11.7 &  9.20 &   25.75 & K3V   & S2 &  30 &   2965 &   $-$73.61 & \ldots & \ldots  \\
HIP 14478    &  03 06 51.34 &  $+$40 21 33.5 &  9.63 &   37.02 & K6    & S1 &  15 &   2917 &   $-$50.87 & \ldots & \ldots  \\
HIP 14669    &  03 09 30.79 &  $+$45 43 57.9 & 10.17 &   57.11 & M2V   & V  &   9 &   2629 &    $-$4.51 &   1.99 &   35.2  \\
HIP 14864    &  03 11 56.83 &  $+$61 31 13.0 & 10.05 &   39.82 & M0Ve  & S2 &  33 &   3023 &   $-$32.10 & \ldots & \ldots  \\
BD+03 480    &  03 28 14.92 &  $+$04 09 47.4 &  9.49 &   11.99 & G0    & C  &  11 &   4764 &    12.66 &   0.57 &    1.1  \\
HIP 17102    &  03 39 48.96 &  $+$33 28 24.3 &  9.05 &   25.49 & K2    & S2 &  23 &   2777 &     4.27 & \ldots & \ldots  \\
GJ 3248      &  03 48 38.24 &  $+$73 32 35.3 & 11.32 &   62.71 & M1V   & V? &  11 &   2971 &    $-$8.08 &   0.78 &    5.0  \\
HIP 18448    &  03 56 36.22 &  $+$69 50 55.9 &  9.33 &    6.71 & K0    & S1 &  29 &   6014 &    16.66 & \ldots & \ldots  \\
HIP 19410    &  04 09 26.37 &  $-$14 41 54.1 & 10.61 &   24.67 & K5V   & V  &   3 &   4350 &     6.34 &   7.97 &   99.0  \\
HIP 19915    &  04 16 19.83 &  $+$36 44 02.8 &  8.98 &    6.01 & F8    & S2 &  41 &  10496 &    $-$8.16 & \ldots & \ldots  \\
HD 279846    &  04 26 09.68 &  $+$34 09 34.2 & 10.50 &   12.14 & K2    & S2 &  28 &   6089 &    12.43 & \ldots & \ldots  \\
HIP 20709    &  04 26 15.05 &  $+$34 42 57.2 &  8.29 &    7.60 & F5    & S2 &  27 &   4743 &    44.76 & \ldots & \ldots  \\
HIP 21710    &  04 39 42.61 &  $+$09 52 19.5 &  9.19 &   36.80 & K2    & S1 &  16 &   1340 &   $-$25.93 & \ldots & \ldots  \\
HIP 21845    &  04 41 47.25 &  $+$28 39 35.9 &  8.85 &    8.70 & F8    & V? &  11 &   5191 &    11.20 &   0.59 &    2.3  \\
HIP 23550    &  05 03 51.96 &  $+$24 58 22.1 &  7.43 &   13.69 & G8V   & V  &  16 &   3271 &    54.18 &   1.18 &   10.6  \\
HIP 24488    &  05 15 15.46 &  $+$47 10 14.6 &  6.92 &    8.73 & G5III & s2 &  10 &   7146 &    24.42 & \ldots & \ldots  \\
GJ 220       &  05 53 14.04 &  $+$24 15 32.9 & 10.82 &   51.50 & M2.0V & V  &  13 &   6089 &    26.45 &   1.75 &   28.2  \\
HIP 28663    &  06 03 08.64 &  $+$14 21 54.4 &  8.31 &    9.74 & F4IV  & S1 &  30 &   1722 &   $-$25.10 & \ldots & \ldots  \\
HIP 29295    &  06 10 34.62 &  $-$21 51 52.7 &  8.12 &  173.70 & M1V   & C  &   6 &   5754 &     4.71 &   0.32 &    0.3  \\
HIP 29316    &  06 10 54.80 &  $+$10 19 05.0 & 10.39 &   91.65 & M2.5V & V  &  10 &   2567 &    52.81 &   1.27 &   15.4  \\
HIP 30269    &  06 22 02.50 &  $-$05 27 17.0 &  8.06 &    3.22 & F5V   & V  &  14 &   5389 &    20.29 &  14.85 &   99.0  \\
HIP 33560    &  06 58 26.05 &  $-$12 59 30.6 &  9.16 &   44.41 & K4V   & V? &  14 &   8376 &    $-$4.33 &   0.96 &    2.3  \\
HIP 34341    &  07 07 09.31 &  $+$03 26 50.7 &  9.87 &   38.26 & K5    & S1 &  21 &   5703 &   $-$17.35 & \ldots & \ldots  \\
HIP 35706    &  07 22 02.05 &  $+$68 16 27.6 & 10.10 &   23.84 & K5V   & S1 &  21 &   5824 &   $-$29.95 & \ldots & \ldots  \\
HIP 36758    &  07 33 34.77 &  $+$39 27 14.0 &  9.75 &    5.95 & F8    & V? &  11 &   1540 &    36.73 &   1.02 &    2.7  \\
HIP 38195    &  07 49 32.01 &  $+$41 28 08.3 &  9.41 &    8.98 & G5    & C? &  10 &   6508 &    71.24 &   1.69 &    7.1  \\
HIP 39681    &  08 06 34.41 &  $+$22 27 24.2 &  7.22 &   14.73 & G5IV  & S1 &  68 &  10984 &    $-$0.57 & \ldots & \ldots  \\
HIP 40253    &  08 13 17.31 &  $+$49 13 15.5 &  8.54 &    8.59 & F5    & S1 &  67 &   6961 &    $-$3.26 & \ldots & \ldots  \\
HIP 40724    &  08 18 44.42 &  $-$15 12 08.5 &  9.87 &   28.85 & K5V   & V  &   2 &    797 &    88.15 &   1.05 &    7.6  \\
HD 71028     &  08 26 07.19 &  $+$28 24 10.7 &  8.01 &    2.21 & K0III & S1 &  29 &   7645 &    34.15 & \ldots & \ldots  \\
HIP 42507    &  08 40 00.27 &  $-$06 28 33.1 &  9.88 &   38.80 & K6V   & C? &   5 &   2245 &   $-$12.14 &   1.38 &   17.1  \\
HIP 42550    &  08 40 22.54 &  $+$51 45 06.6 &  7.70 &    1.70 & G5III & C  &  11 &  10684 &  $-$101.16 &   0.44 &    1.3  \\
HD 73394B    &  08 40 18.25 &  $+$51 45 46.8 & 11.54 &    1.41 & --    & s2 &   5 &   4133 &   $-$32.54 & \ldots & \ldots  \\
HIP 43820    &  08 55 24.82 &  $+$70 47 39.2 &  8.61 &   86.32 & M1V   & V  &  19 &   5226 &    44.64 & \ldots & \ldots  \\
HD 75632B    &  08 55 24.82 &  $+$70 47 39.2 &  8.86 &   86.32 & M1V   & C  &   2 &    326 &    43.81 &   0.08 &    0.3  \\
HIP 46383    &  09 27 28.37 &  $+$39 30 17.9 &  9.85 &   30.60 & K4V   & S2 &  12 &   2585 &   $-$32.36 & \ldots & \ldots  \\
BD-08 2689   &  09 28 51.52 &  $-$09 16 00.8 & 10.54 &    9.20 & M0V   & V  &   4 &   2208 &   $-$14.81 &   1.55 &   24.5  \\
HIP 46926    &  09 33 52.46 &  $+$15 29 31.2 &  9.47 &    9.32 & G0    & S2 &  38 &   5046 &   $-$10.86 & \ldots & \ldots  \\
HIP 47133    &  09 36 15.91 &  $+$37 31 45.5 & 11.02 &   25.78 & M0V   & S2 &  16 &   5819 &    $-$0.68 & \ldots & \ldots  \\
HIP 47899    &  09 45 44.26 &  $+$50 14 08.3 & 11.19 &   12.58 & K4V   & S2 &  30 &   6588 &   $-$15.01 & \ldots & \ldots  \\
HIP 48346    &  09 51 18.98 &  $+$37 36 15.9 &  9.96 &   19.28 & K8    & S2 &  23 &   2828 &   $-$14.65 & \ldots & \ldots  \\
HIP 50156    &  10 14 19.18 &  $+$21 04 29.6 & 10.08 &   42.74 & M0.7V & S1 &  13 &   2527 &     8.74 & \ldots & \ldots  \\
HIP 50271    &  10 15 52.67 &  $+$25 50 01.2 &  9.44 &    5.77 & G0    & S1 &  49 &  10619 &     4.29 & \ldots & \ldots  \\
HIP 52021    &  10 37 47.41 &  $-$06 23 22.5 &  9.94 &   26.41 & K8    & V  &   8 &   6592 &   $-$11.58 &   7.11 &   99.0  \\
HIP 54002    &  11 02 50.12 &  $-$09 19 49.3 &  9.04 &   32.07 & K3V   & V  &   6 &   6554 &    $-$6.78 &   0.98 &    9.4  \\
HIP 54094    &  11 04 07.16 &  $+$53 22 55.5 &  9.98 &   21.45 & ?     & V? &   9 &   6554 &   $-$23.88 &   0.58 &    4.2  \\
HIP 56229    &  11 31 36.39 &  $+$40 30 01.2 &  9.75 &   22.85 & M0    & S2 &   8 &    473 &    12.02 & \ldots & \ldots  \\
HIP 57058    &  11 41 49.59 &  $+$05 08 26.5 &  9.59 &   32.26 & K4V   & S1 &  11 &   2602 &    18.90 & \ldots & \ldots  \\
BD+44 2120A  &  11 43 48.16 &  $+$44 10 46.5 & 11.22 &    2.86 & F5    & C  &   5 &   4136 &    $-$5.73 &   0.74 &    3.6  \\
BD+44 2120B  &  11 43 47.90 &  $+$44 10 40.3 & 11.45 &    3.06 & ?     & S1 &  17 &   4136 &    $-$4.39 & \ldots & \ldots  \\
BD+44 2120C  &  11 43 44.06 &  $+$44 10 49.1 & 11.04 &    3.06 & ?     & C  &  11 &   7654 &    15.01 &   0.57 &    0.6  \\
GQ Leo       &  11 47 45.73 &  $+$12 54 03.4 & 10.83 &   16.29 & K5Ve  & C  &  12 &   5468 &   $-$12.77 &   1.31 &   15.0  \\
HIP 57857    &  11 51 56.21 &  $+$33 07 11.4 & 10.97 &   18.50 & K0V   & V  &  11 &   6645 &   $-$20.28 &   2.96 &   95.6  \\
HIP 57949    &  11 53 05.24 &  $+$18 55 48.1 & 11.73 &   32.00 & M0.5V & V  &   7 &   5529 &     6.82 &   2.48 &   33.2  \\
HIP 59000    &  12 05 50.66 &  $-$18 52 30.9 & 10.02 &   42.72 & K5V   & -  &   1 &      0 &    $-$8.20 & \ldots & \ldots  \\
HIP 60433    &  12 23 26.85 &  $+$20 17 27.0 & 10.02 &   24.99 & K4V   & V  &  15 &   6594 &   $-$40.01 &   6.20 &   99.0  \\
HIP 60448    &  12 23 34.71 &  $+$27 54 47.6 & 11.41 &   33.82 & K5V   & V  &   5 &   6592 &   $-$31.14 &   1.39 &   22.8  \\
HIP 61436    &  12 35 19.72 &  $+$34 04 06.6 & 10.51 &   24.43 & K5V   & S2 &  24 &   2671 &    $-$0.01 & \ldots & \ldots  \\
HIP 62505    &  12 48 32.31 &  $-$15 43 10.1 &  7.89 &   39.21 & K2.5V & V  &  12 &   4417 &    $-$1.87 &   3.35 &   32.9  \\
HIP 62755    &  12 51 34.58 &  $+$59 50 25.9 & 11.31 &    0.81 & K?    & S1 &  11 &   3000 &   $-$47.03 & \ldots & \ldots  \\
HIP 63253    &  12 57 40.21 &  $+$35 13 30.1 & 10.68 &   46.84 & M0V   & V  &  11 &   2615 &   $-$10.00 &   1.32 &   25.7  \\
HIP 63816    &  13 04 46.60 &  $+$55 54 10.1 & 10.75 &   30.63 & M0V   & C  &   3 &   2598 &   $-$22.47 &   0.32 &    1.6  \\
HIP 63942    &  13 06 15.40 &  $+$20 43 45.3 &  9.40 &   53.18 & K4V   & C  &  13 &   5545 &    $-$2.84 &   0.57 &    1.3  \\
HIP 65012    &  13 19 34.69 &  $+$35 06 24.5 & 11.90 &   73.99 & M3V   & -  &   1 &      0 &    $-$5.20 & \ldots & \ldots  \\
HIP 65026    &  13 19 45.65 &  $+$47 46 41.0 &  8.76 &  109.98 & M2V   & S2 &  27 &   2629 &     0.12 & \ldots & \ldots  \\
HIP 65327    &  13 23 23.30 &  $+$57 54 22.1 &  9.56 &   41.47 & K5V   & S1 &  15 &   6115 &    $-$8.53 & \ldots & \ldots  \\
GJ 513       &  13 29 21.31 &  $+$11 26 26.5 & 11.92 &   52.30 & M3V   & V  &   4 &    416 &    29.55 &   2.73 &    8.5  \\
HIP 65887    &  13 30 22.60 &  $+$07 24 54.5 &  7.63 &    3.29 & K0    & S1 &  25 &   3674 &    $-$3.42 & \ldots & \ldots  \\
HIP 66290    &  13 35 11.42 &  $+$22 29 59.0 &  6.99 &   26.29 & F5V   & S1 &  36 &   8395 &   $-$14.04 & \ldots & \ldots  \\
HIP 67086    &  13 45 02.39 &  $+$02 05 31.5 & 10.78 &   21.67 & K5    & C? &  14 &   2886 &   $-$27.23 & \ldots & \ldots  \\
BD+26 2498   &  13 49 18.69 &  $+$25 52 54.2 &  9.85 &    1.40 & G5    & S1 &  31 &   6654 &   $-$13.64 & \ldots & \ldots  \\
HIP 67808    &  13 53 27.56 &  $+$12 56 33.4 &  9.77 &   45.62 & K7V   & V? &   6 &   2659 &   $-$18.71 &   0.43 &    2.2  \\
BD+19 2735   &  13 58 13.62 &  $+$19 17 11.8 &  9.31 &   27.17 & K2    & S1 &  20 &   5133 &    $-$9.53 & \ldots & \ldots  \\
HIP 68801    &  14 05 03.72 &  $+$10 00 48.9 &  8.68 &   19.58 & G5    & S2 &  24 &   5429 &   $-$36.32 & \ldots & \ldots  \\
HIP 69549    &  14 14 12.16 &  $+$18 05 06.8 &  7.98 &   11.72 & G     & S2 &  29 &   6951 &     8.58 & \ldots & \ldots  \\
HIP 71904    &  14 42 26.26 &  $+$19 30 12.7 & 10.03 &   42.24 & K5V   & C  &   2 &   2550 &   $-$28.08 &   0.09 &    0.2  \\
HIP 71914    &  14 42 33.81 &  $+$19 28 48.6 &  9.12 &   41.70 & K5V   & -  &   1 &      0 &   $-$28.70 & \ldots & \ldots  \\
HIP 72508    &  14 49 32.38 &  $+$51 22 28.2 &  6.48 &   19.09 & F5IV  & s2 &  11 &   7052 &    $-$6.13 & \ldots & \ldots  \\
BD+49 2364   &  15 13 25.00 &  $+$49 00 24.0 & 10.77 &    0.97 & ?     & V  &  22 &  10789 &   $-$74.33 &   1.69 &   19.7  \\
HIP 76941    &  15 42 38.57 &  $+$31 56 45.5 & 10.88 &   20.10 & K5V   & S1 &  26 &   2886 &   $-$12.50 & \ldots & \ldots  \\
HIP 77141    &  15 45 00.29 &  $+$35 57 40.9 & 10.11 &   18.50 & K4/5V & S1 &  30 &   2913 &    $-$3.46 & \ldots & \ldots  \\
HIP 78158    &  15 57 33.88 &  $+$34 32 22.8 & 10.83 &   19.30 & K5V   & S1 &  19 &   2748 &   $-$44.84 & \ldots & \ldots  \\
HIP 79796    &  16 17 05.39 &  $+$55 16 09.1 &  9.46 &   49.35 & M1.5V & S1 &  14 &   2895 &   $-$30.82 &  12.49 &   99.0  \\
HIP 80751    &  16 29 14.36 &  $+$23 46 33.9 & 10.08 &   30.84 & K5V   & S1 &  14 &   6554 &   $-$32.81 & \ldots & \ldots  \\
BD+52 1968A  &  16 39 13.76 &  $+$52 37 39.4 & 10.01 &   22.86 & K8    & V  &  13 &   2926 &    $-$8.55 &   3.30 &   99.0  \\
BD+52 1968B  &  16 39 13.10 &  $+$52 37 38.2 & 11.40 &   22.71 & --    & C  &   2 &      0 &    $-$8.69 &   0.39 &    6.9  \\
HIP 82506    &  16 51 46.46 &  $+$25 24 00.7 &  7.09 &   14.84 & F4III & V  &   8 &   4785 &   $-$25.39 &   4.76 &   99.0  \\
BD+61 1678C  &  17 35 34.49 &  $+$61 40 53.6 &  9.97 &   69.83 & M1V   & C  &   9 &   3105 &   $-$15.33 &   0.75 &    2.1  \\
HIP 86221    &  17 37 10.77 &  $+$27 53 47.2 &  9.20 &   32.00 & M0V   & C  &   2 &   2825 &   $-$42.55 &   0.33 &    3.3  \\
BD+27 2853C  &  17 37 11.41 &  $+$27 53 51.4 & 11.61 &   31.09 & K5    & -  &   1 &      0 &   $-$43.39 & \ldots & \ldots  \\
HIP 90274    &  18 25 10.11 &  $+$64 50 18.3 &  6.86 &    5.70 & K0    & s2 &  28 &   5881 &   $-$52.07 & \ldots & \ldots  \\
HIP 91043    &  18 34 20.10 &  $+$18 41 24.2 &  7.45 &   28.27 & G2V   & s2 &  39 &   4879 &   $-$22.21 & \ldots & \ldots  \\
HIP 92952    &  18 56 15.93 &  $+$54 31 48.1 & 10.37 &   21.51 & M0V   & S1 &  27 &   2944 &   $-$18.38 & \ldots & \ldots  \\
HIP 94557    &  19 14 39.16 &  $+$19 19 03.7 & 11.54 &   55.24 & M4.5V & V  &   3 &   2904 &    $-$4.28 &  19.34 &   99.0  \\
HIP 94622    &  19 15 18.84 &  $+$24 53 49.5 &  9.78 &   34.57 & M0    & s2 &   7 &   2989 &   $-$72.83 & \ldots & \ldots  \\
BD+77 767    &  20 11 00.50 &  $+$77 43 18.4 & 10.30 &   24.54 & K8    & S1 &  18 &   2822 &   $-$25.83 & \ldots & \ldots  \\
HIP 99969    &  20 16 55.43 &  $+$06 55 18.3 &  9.47 &   22.67 & K4V   & s2 &   8 &   2611 &   $-$56.38 & \ldots & \ldots  \\
HIP 101941   &  20 39 29.75 &  $+$28 05 18.6 &  7.78 &    2.63 & K4III & S1 &  46 &   4775 &   $-$20.56 & \ldots & \ldots  \\
HIP 102300   &  20 43 41.37 &  $+$64 16 54.1 & 11.38 &   46.53 & M0Ve  & V  &   5 &   2963 &    15.51 &   1.25 &   11.8  \\
HIP 102320   &  20 43 53.36 &  $+$31 19 10.4 &  9.96 &   24.06 & K5    & S2 &  29 &   3013 &   $-$21.08 & \ldots & \ldots  \\
HIP 102718   &  20 48 50.72 &  $+$05 11 58.8 &  9.69 &    9.70 & F7Vw  & C? &   6 &   4290 &  $-$117.67 &   0.64 &    2.8  \\
HIP 103375   &  20 56 37.80 &  $+$52 49 36.9 &  9.66 &    7.55 & G0    & C? &  11 &   4418 &   $-$47.55 &   0.53 &    2.5  \\
HIP 104994   &  21 15 54.95 &  $+$28 57 47.4 & 10.41 &    6.97 & G5    & S3 &  30 &   6669 &   $-$46.87 & \ldots & \ldots  \\
HIP 105504   &  21 22 07.78 &  $-$10 30 47.9 & 10.33 &   24.00 & K7    & V  &   5 &   2613 &     7.40 &  17.45 &   99.0  \\
BD+47 3439   &  21 30 48.00 &  $+$48 27 25.4 &  8.66 &    7.12 & K0    & s2 &  14 &   5465 &    10.04 & \ldots & \ldots  \\
HIP 110291   &  22 20 23.85 &  $+$46 25 05.7 &  8.51 &   16.12 & G0    & S1 &  40 &   1571 &  $-$108.04 & \ldots & \ldots  \\
HIP 110526   &  22 23 29.10 &  $+$32 27 33.9 & 10.76 &   64.47 & M3.0V & C  &  13 &   2940 &   $-$19.90 &   0.52 &    2.4  \\
HIP 110978   &  22 29 04.21 &  $-$13 42 01.8 &  9.17 &    1.25 & K2III & V? &   3 &     34 &    $-$1.37 &   0.82 &    6.3  \\
HIP 111685   &  22 37 29.90 &  $+$39 22 51.6 &  9.41 &   41.99 & M0Ve  & S1 &  10 &   5457 &   $-$58.38 & \ldots & \ldots  \\
HIP 111942   &  22 40 30.30 &  $+$43 00 47.4 &  9.83 &   31.92 & K8V   & S1 &  20 &   2940 &   $-$31.76 & \ldots & \ldots  \\
HIP 112040   &  22 41 34.99 &  $+$18 49 27.5 & 10.51 &   31.85 & M0V   & V  &  13 &   5469 &   $-$15.94 &   1.17 &   10.9  \\
HIP 112268   &  22 44 24.92 &  $+$17 33 23.8 & 10.19 &   19.83 & K6V   & V  &  13 &   5521 &   $-$38.11 &   0.95 &    8.7  \\
HIP 112523   &  22 47 30.45 &  $+$19 13 27.4 & 10.29 &   26.95 & K5V   & S1 &  13 &   5458 &     3.97 &   1.86 &   28.7  \\
HIP 116003   &  23 30 13.44 &  $-$20 23 27.5 & 11.11 &   62.67 & M2Ve  & V  &   2 &      7 &    $-$6.83 &   7.07 &   91.2  \\
BD+66 1664   &  23 58 10.67 &  $+$67 33 59.7 &  8.73 &   11.13 & G5    & S1 &  33 &   1175 &   $-$22.08 & \ldots & \ldots  \\
HIP 118212   &  23 58 43.51 &  $+$46 43 44.9 &  9.62 &   58.41 & K7V   & S1 &  18 &   2986 &     1.00 & \ldots & \ldots  \\

